High-Performance Permanent Magnet Array Design by a Fast Genetic Algorithm (GA)-based Optimization for Low-Field Portable MRI

A permanent magnet array (PMA) is a preferred source of magnetic field for body-part-dedicated low-field (<0.5 T) portable magnetic resonance imaging (MRI) because it has a small footprint, no power consumption, and no need for a cooling system. The current popular PMA is limited by the transversal field below 100 mT, where advanced technologies developed for the long-bore MRI systems (e.g., multi-channel techniques) cannot be applied. In this paper, a sparse high-performance PMA is proposed based on inward-outward ring pairs and using magnet blocks that can be bought off the shelf, targeting on portable head imaging. Through a fast genetic algorithm (GA)-based optimization, the proposed PMA has a longitudinal magnetic field with an average field strength of 111.40 mT and a monotonic field pattern with inhomogeneity of 10.57 mT (an RF bandwidth of <10%) within a Field of View (FoV) of 20 cm in diameter and 4.5 cm in length. The resulting field was validated using analytic calculations and numerical simulations. The encoding capability of the designed PMA was examined by checking the quality of the simulated reconstructed images. The proposed field outperforms a linear pattern for encoding. The PMA is 57.91 cm wide, 38 cm long, has a 5-gauss range of 87x87x104 cm^3, allowing an operation in a small space. It weights 126.08kg, comprising of a stationary main array that supplies a strong homogeneous field, and a light rotatable sub-gradient-array (5.12kg) that supplies a monotonic field for signal encoding. It has a magnetic field generation efficiency of 0.88mT/kg, the highest among sparse PMAs that offer a monotonic field pattern. The force experienced by each magnet was calculated to validate the feasibility of physical implementation. The proposed PMA can be a promising alternative to supply the main and gradient fields combined for dedicated portable MRI.

==> fig_accel_approach.tex <==
\begin{figure}[t]
\centering
\begin{center}
%\includegraphics[width=1\linewidth]{figures/Fig_accel_approach.jpg}\\
\newcommand{\patchSize}{2.45cm}
\scriptsize
\setlength\tabcolsep{0.1cm}
\includegraphics[width=0.75\linewidth]{figures/acc_1.jpg}\\
(a)\\
\includegraphics[width=0.75\linewidth]{figures/acc_2.jpg}\\
(b)\\
\end{center}
\caption{The illustration of (a) Approach-1 and (b) Approach-2 for acceleration of calculation of the magnetic fields of PMAs.}
\label{fig:accel_approach}
\end{figure}

==> fig_axial.tex <==
\begin{figure}[t]
\centering
\begin{center}
		\newcommand{\patchSize}{2.45cm}
		\scriptsize
		\setlength\tabcolsep{0.1cm}
    % 	\hspace{0.001\linewidth}
        \includegraphics[width=0.65\linewidth]{figures/Fig_BxBy_1.jpg}\\
        \hspace{0.01\linewidth}(a)\hspace{0.3\linewidth}(b)\hspace{0.5\linewidth}\\
        \includegraphics[width=0.65\linewidth]{figures/Fig_BxBy_2.jpg}\\
        \hspace{0.01\linewidth}(c)\hspace{0.3\linewidth}(d)\hspace{0.5\linewidth}\\
\end{center}
% \includegraphics[width=\linewidth]{stream}
\caption{(a) x-component ($B_x$), (b) y-component ($B_y$), (c) the ratio ($B_x/B_z$), and (d) the ratio ($B_y/B_z$) of the optimized field pattern on the slice $z=7.5$ mm.}
\label{fig:axial}
\end{figure}

==> fig_coord_trans.tex <==
\begin{figure}[t]
\centering
\begin{center}
\newcommand{\patchSize}{2.45cm}
\scriptsize
\setlength\tabcolsep{0.1cm}
\includegraphics[width=1\linewidth]{figures/Fig_coord_trans.jpg}\\
\hspace{0.05\linewidth}(a)\hspace{0.45\linewidth}(b)\hspace{0.25\linewidth}\\    	
\end{center}
\caption{Illustration and equations of the coordinate transformation for the calculation of magnetic fields of a $y$-polarized block.}
\label{fig:coord_trans}
\end{figure}

==> fig_forLoop.tex <==
\begin{figure}[t]
\centering
\begin{center}
%\includegraphics[width=1\linewidth]{figures/Fig_accel_approach.jpg}\\
\includegraphics[width=0.8\linewidth]{figures/nested_for.jpg}\\
\end{center}
\caption{The illustration of nested for-loop approach of calculation of the magnetic fields of PMAs.}
\label{fig:forLoop}
\end{figure}

==> fig_magnet_base_case.tex <==
\begin{figure}[]
\centering
\begin{center}
\newcommand{\patchSize}{2.45cm}
\scriptsize
\setlength\tabcolsep{0.1cm}
\includegraphics[width=1\linewidth]{figures/magnet_blocks.jpg}\\
\hspace{0.05\linewidth}(a)\hspace{0.5\linewidth}(b)\\    
\end{center}
\caption{Single magnet blocks with (a) $y$-polarization and (b) $z$-polarization.}
\label{fig:block_base_case}
\end{figure}

==> fig_sim_cal_comp.tex <==
\begin{figure}[t]
\centering
\begin{center}
		\newcommand{\patchSize}{2.45cm}
		\scriptsize
		\setlength\tabcolsep{0.1cm}
    % 	\hspace{0.001\linewidth}
        \includegraphics[width=1\linewidth]{figures/Fig_sim_cal_1.jpg}\\
        (a)\hspace{0.3\linewidth}(b)\hspace{0.3\linewidth}(c)\\
        \includegraphics[width=1\linewidth]{figures/Fig_sim_cal_2.jpg}\\
        (d)\hspace{0.3\linewidth}(e)\hspace{0.3\linewidth}(f)\\
        \includegraphics[width=1\linewidth]{figures/Fig_sim_cal_3.jpg}\\
        (g)\hspace{0.3\linewidth}(h)\hspace{0.3\linewidth}(i)\\
\end{center}
% \includegraphics[width=\linewidth]{stream}
\caption{(a)-(c) CST simulation, (d)-(f) Matlab calculation and (g)-(i) the difference between calculation and simulation of the field patterns produced by the base, shimming, and sub-gradient array.}
\label{fig:cal_sim_comp}
\end{figure}

==> tab_parameters.tex <==
\begin{table}[htbp]
   \small % text size of table content
   \centering % center the table
   \begin{tabular}{lccr} % alignment of each column data
   \toprule[\heavyrulewidth]\toprule[\heavyrulewidth]
   \textbf{Sub Array Name} & \textbf{Parameter Name} & \textbf{Parameter Value} & \textbf{Unit} \\ 
   \midrule
   \multirow{4}{*}{IO Ring Pair}
   & $a_{base}$ & 120 & \si{\milli\meter} \\
   & $b_{base}$ & 30 & \si{\milli\meter}\\
   & $h_{base}$ & 90 & \si{\milli\meter}\\
   & $N_{\Theta, \text{base}}$ & 24 & / \\
   \midrule
   \multirow{3}{*}{Shimming Array}
   & $a_{shim}$ & 10 & \si{\milli\meter}\\
   & $N_{\Theta, \text{shim}}$ & 36 & / \\
   & $N_{\text{Z, shim}}$ & 30 & / \\
   \midrule
   \multirow{2}{*}{Sub-Gradient Array}
   & $N_{\Theta, \text{g}}$ & 36 & / \\
   & $\Delta x$ & 8 & \si{\milli\meter}\\
   \midrule
   \multirow{3}{*}{Iron Bars}
   & $a_{iron}$ & 10 & \si{\milli\meter}\\
   & $b_{iron}$ & 20 & \si{\milli\meter}\\
   & $h_{iron}$ & 400 & \si{\milli\meter}\\
   \bottomrule[\heavyrulewidth] 
   \end{tabular}
   \caption{\label{tab:predefined_parameters} Predefined parameters for the magnet array.}
\end{table}
   
\begin{table}[htbp]
   \small % text size of table content
   \centering % center the table
   \begin{tabular}{lcccr} % alignment of each column data
   \toprule[\heavyrulewidth]\toprule[\heavyrulewidth]
   \textbf{Sub Array Name} & \multicolumn{2}{c}{\textbf{Parameter Name}} & \multicolumn{2}{c}{\textbf{Parameter Value}} \\
   \midrule
   &&&\textbf{Yokeless Case} & \textbf{Yoked Case}\\
   \multirow{2}{*}{IO Ring Pair} & \multicolumn{2}{c}{$R'_{base}$} & \multicolumn{2}{c}{237\si{\milli\meter}} \\
   & \multicolumn{2}{c}{$Z'_{base}$} & \multicolumn{2}{c}{155 \si{\milli\meter}}\\
   \midrule
   \multirow{15}{*}{Shimming Array} &
   \multirow{15}{*}{ \rotatebox[origin=c]{90}{Direction, Remanence}}
   & 1 & z+, 1.188 \si{\tesla} & z+, 1.188 \si{\tesla}\\
   && 2 & in/out, 1.4 \si{\tesla} & z+, 1.188 \si{\tesla}\\
   && 3 & z-, 1.188 \si{\tesla} & in/out, 1.188 \si{\tesla}\\
   && 4 & in/out, 1.4 \si{\tesla} & Empty \\
   && 5 & out/in, 1.188 \si{\tesla} & z+, 1.4 \si{\tesla}\\
   && 6 & out/in, 1.188 \si{\tesla} & out/in, 1.4 \si{\tesla}\\
   && 7 & out/in, 1.4 \si{\tesla} & out/in, 1.188 \si{\tesla}\\
   && 8 & out/in, 1.188 \si{\tesla} & out/in, 1.188 \si{\tesla}\\
   && 9 & z-, 1.188 \si{\tesla} & out/in, 1.188 \si{\tesla}\\
   && 10 & z-, 1.4 \si{\tesla} & out/in, 1.4 \si{\tesla}\\
   && 11 & z-, 1.188 \si{\tesla} & out/in, 1.188 \si{\tesla}\\
   && 12 & Empty & z-, 1.188 \si{\tesla}\\
   && 13 & z-, 1.4 \si{\tesla} & in/out, 1.188 \si{\tesla}\\
   && 14 & z-, 1.4 \si{\tesla} & z-, 1.4 \si{\tesla}\\
   && 15 & z-, 1.4 \si{\tesla} & z-, 1.4 \si{\tesla}\\
   \midrule
   Sub-gradient Array & \multicolumn{2}{c}{$h_g$} & 100\si{\milli\meter} & 90\si{\milli\meter}\\
   
   \bottomrule[\heavyrulewidth] 
   \end{tabular}
   \caption{\label{tab:optimzed_parameters} Optimized parameters for both yoked and yokeless magnet array. }
\end{table}
